Towards a Standardised Performance Evaluation Protocol for Cooperative MARL

Multi-agent reinforcement learning (MARL) has emerged as a useful approach to solving decentralised decision-making problems at scale. Research in the field has been growing steadily with many breakthrough algorithms proposed in recent years. In this work, we take a closer look at this rapid development with a focus on evaluation methodologies employed across a large body of research in cooperative MARL. By conducting a detailed meta-analysis of prior work, spanning 75 papers accepted for publication from 2016 to 2022, we bring to light worrying trends that put into question the true rate of progress. We further consider these trends in a wider context and take inspiration from single-agent RL literature on similar issues with recommendations that remain applicable to MARL. Combining these recommendations, with novel insights from our analysis, we propose a standardised performance evaluation protocol for cooperative MARL. We argue that such a standard protocol, if widely adopted, would greatly improve the validity and credibility of future research, make replication and reproducibility easier, as well as improve the ability of the field to accurately gauge the rate of progress over time by being able to make sound comparisons across different works. Finally, we release our meta-analysis data publicly on our project website for future research on evaluation: https://sites.google.com/view/marl-standard-protocol

==> emarl - meta analysis 2/sections/0-abstract.tex <==
\begin{abstract}
Multi-agent reinforcement learning (MARL) has emerged as a useful approach to solving decentralised decision-making problems at scale. Research in the field has been growing steadily with many breakthrough algorithms proposed in recent years. In this work, we take a closer look at this rapid development with a focus on evaluation methodologies employed across a large body of research in cooperative MARL. By conducting a detailed meta-analysis of prior work, spanning 75 papers accepted for publication from 2016 to 2022, we bring to light worrying trends that put into question the true rate of progress. We further consider these trends in a wider context and take inspiration from single-agent RL literature on similar issues with recommendations that remain applicable to MARL. Combining these recommendations, with novel insights from our analysis, we propose a standardised performance evaluation protocol for cooperative MARL. We argue that such a standard protocol, if widely adopted, would greatly improve the validity and credibility of future research, make replication and reproducibility easier, as well as improve the ability of the field to accurately gauge the rate of progress over time by being able to make sound comparisons across different works. Finally, we release our meta-analysis data publicly on our project website for future research on evaluation: \href{https://sites.google.com/view/marl-standard-protocol/}{https://sites.google.com/view/marl-standard-protocol}
\end{abstract}

% Abstract (What-Why-How) \\
% This Paper presents the first (large) meta-analysis of MARL Algorithm papers.\\
% Our analysis is based on 114 research wpapers published from 2015 to 2022.\\
% What we do in the analysis. \\-> collection of MARL papers -> collection of reported MARL algorithm evaluations i.e. details about metrics, details on environments/tasks, the use of confidence, metric and CI values, number of seeds, number of runs, evaluation frequency and duration
% From this we mine the data to find:/Our study shows how:
% describes the state of MARL research procedures, performs algorithm comparisons acrsoss papers\\
% Mention major issues with MARL papers\\
% Briefly describe the guideline we propose\\
% Mention goal of research - to establish better protocols for empirical evaluation of coop MARL algorithms\\
%  reevaluation using PyMARL and SMAC using new protocol



% Due to the potential advantages of the field, Multi-Agent Reinforcement Learning (MARL) has witnessed significant growth and has become a prominent topic in recent years. However, whenever a field has rapid growth in a short time, it frequently encounters a lot of chaos and a lack of regulation and uniformity. To avoid falling in this dilemma to when it comes to evaluation in the MARL experiments, this paper proposes the first major meta-analysis of MARL publications, including 114 research papers manually annotated from 2015 to 2022. (Highlighting some insights)

==> emarl - meta analysis 2/sections/1-introduction.tex <==
\section{Introduction} % NEED TO ADD FOOTNOTE ABOUT SARL -> RL

Empirical evaluation methods in single-agent reinforcement learning (RL)\footnote{In this paper, we use the term "RL" to exclusively refer to \emph{single-agent} RL, as opposed to RL as a field of study, of which MARL is a subfield.} have been closely scrutinised in recent years \citep{IslamReproducibility2017, Machado2017, MSc-2017-Henderson, Zhang2018, henderson2019deep,colas2018random, colas2019hitchhikers, chan-2020-measuringReliability, jordan2020evaluating, engstrom2020implementation, agarwal2022deep}. In this context, the impact of a lack of rigour and methodological standards has already been observed. Fortunately, just as these issues have arisen and been identified, they have also been accompanied by suggested solutions and recommendations from these works. 

Multi-agent reinforcement learning (MARL) extends RL with capabilities to solve large-scale decentralised decision-making tasks where many agents are expected to coordinate to achieve a shared objective \citep{MARL, ReviewCoopMARL-2019-Oroojlooyjadid,GameTheoryMARLOverviewYang}. In this cooperative setting, where there is a common goal and rewards are shared between agents, sensible evaluation methodology from the single-agent case often directly translates to the multi-agent case. However, despite MARL being far less developed and entrenched than RL, arguably making adoption of principled evaluation methods easier, the field remains affected by many of the same issues as found in RL. Implementation variance, inconsistent baselines, and insufficient statistical rigour still affect the quality of reported results. Although work specifically addressing these issues in MARL have been rare, there have been recent publications that implicitly observe some of the aforementioned issues and attempt to address their symptoms but arguably not their root cause \citep{SurpisingPPO-ChaoYu-2021, papoudakis2021benchmarking, hu2022rethinking}. These works usually attempt to perform new summaries of performance or look into the code-level optimisations used in the literature to provide insight into the current state of research. 

In this paper, we argue that to facilitate long-term progress in future research, MARL could benefit from the literature found in RL on evaluation. The highlighted issues and recommendations from RL may serve as a guide towards diagnosing similar issues in MARL, as well as providing scaffolding around which a standardised protocol for evaluation could be developed. In this spirit, we survey key works in RL over the previous decade, each relating to a particular aspect of evaluation, and use these insights to inform potential standards for evaluation in MARL. 

For each aspect of evaluation considered, we provide a detailed assessment of the corresponding situation in MARL through a meta-analysis of prior work. In more detail, our meta-analysis involved manually annotating MARL evaluation methodologies found in research papers published between 2016 to 2022 from various conferences including NeurIPS, ICML, AAMAS and ICLR, with a focus on \textit{deep} cooperative MARL (see Figure \ref{fig: number_of_papers}). In total, we collected data from 75 cooperative MARL papers accepted for publication. Although we do not claim our dataset to comprise the entire field of modern deep MARL, to the best of our knowledge, our data includes all popular and recent deep MARL algorithms and methodologies from seminal papers. We believe this dataset is the first of its kind and we have made it publicly available for further analysis.

\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    % \includegraphics[width=0.4\textwidth, bb=0 0 0 0]
    \includegraphics[width=0.5\textwidth]{figures/main/number_of_papers_by_year-crop.pdf}
    \caption{Recorded papers by year in the meta-analysis on evaluation methodologies in cooperative MARL.}
    \label{fig: number_of_papers}
\end{wrapfigure}

By mining the data on MARL evaluation from prior work, we highlight how certain trends, worrying inconsistencies, poor reporting, a lack of uncertainty estimation, and a general absence of proper standards for evaluation, is plaguing the current state of MARL research, making it difficult to draw sound conclusions from comparative studies. We combine these findings with the earlier issues and recommendations highlighted in the literature on RL evaluation, to propose a standardised performance evaluation protocol for cooperative MARL research. 

In addition to a standardised protocol for evaluation, we expose trends in the use of benchmark environments and suggest useful standards for environment designers that could further improve the state of evaluation in MARL. We touch upon aspects of environment bias, manipulation, level/map cherry picking as well as scalability and computational considerations. Our recommendations pertain to designer specified standards concerning the use of a particular environment, its agreed upon settings, scenarios and version, as well as improved reporting by authors and preferring the use of environments designed to test generalisation. 

There are clear parallels between RL and MARL evaluation, especially in the cooperative setting. Therefore, we want to emphasise that our contribution in this work is less focused on innovations in protocol design (of which much can be ported from RL) and more focused on data-driven insights on the current state of MARL research and a proposal of standards for MARL evaluation.  

% TODO: Stress the limitation here



==> emarl - meta analysis 2/sections/10-checklist.tex <==
\section*{Checklist}

\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
  \answerYes{}
  \item Did you describe the limitations of your work?
  \answerYes{We did this both in our introduciton and conclusion.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{We did not find this necessary given the nature of the work.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
  \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
      \item Did you state the full set of assumptions of all theoretical results?
  \answerNo{}
      \item Did you include complete proofs of all theoretical results?
    \answerNo{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
  \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
  \answerYes{See supplementary material.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{In main text and for experiments in supplementary material.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
   \answerYes{See supplementary material.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
  \answerNo{Links to repositories were given where the license can be found.}
  \item Did you include any new assets either in the supplemental material or as a URL?
  \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
  \answerNo{All collected data is publicaly available, accesilble via open-access publication.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
  \answerNo{The meta-analysis data contains information typical to any research meta-analysis, including author information, paper titles and information extracted from each paper.}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
  \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
  \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
  \answerNA{}
\end{enumerate}


\end{enumerate}

==> emarl - meta analysis 2/sections/2-eval-rl-marl.tex <==
\section{From RL to MARL evaluation: lessons, trends and recommendations} 

In this section, we provide a list of key lessons from RL that are applicable to MARL evaluation. We highlight important issues identified from the literature on RL evaluation, and for each issue, provide an assessment of the corresponding situation and trends in MARL. Finally, we conclude each lesson with recommendations stemming from our analysis and the literature. 

% Based on the insights and recommendations from this section, we proceed with our suggested standardised performance evaluation protocol in Section \ref{sec: eval protocol}. 

\subsection{Lesson 1: Know the true source of improvement and report everything}

 \textbf{Issue in RL} -- \textit{Confounding code-level optimisations and poor reporting}: It has been shown empirically that across some RL papers there is considerable variance in the reported results for the same algorithms evaluated on the same environments \citep{henderson2019deep, jordan2020evaluating}. This variance impedes the development of novel algorithmic developments by creating misleading performance comparisons and making direct comparisons of results across papers difficult. Implementation and code-level optimisation differences can have a significant impact on algorithm performance and may act as confounders during performance evaluation \citep{engstrom2020implementation,andrychowicz2020matters}. It is rare that these implementation and code-level details are reported, or that appropriate ablations are conducted to pinpoint the true source of performance improvement.

\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.02\textwidth}
        \scriptsize
        \textbf{(a)}
    \end{subfigure}
    \begin{subfigure}[t]{0.28\textwidth}
        \includegraphics[width=\linewidth, valign=t]{figures/main/1_algos_used_per_year-crop.pdf}
    \end{subfigure}
    \hspace{1mm}
    \begin{subfigure}[t]{0.02\textwidth}
        \scriptsize
        \textbf{(b)}
    \end{subfigure}
    \begin{subfigure}[t]{0.58\textwidth}
        \includegraphics[width=\linewidth, valign=t]{figures/main/distribution_qmix_smac-crop.pdf}
    \end{subfigure}

    \vspace{0.4cm}

    \begin{subfigure}[t]{0.02\textwidth}
        \scriptsize
        \textbf{(c)}
    \end{subfigure}
    \begin{subfigure}[t]{0.45\textwidth}
        \includegraphics[width=\linewidth, valign=t]{figures/main/qmix_MMM2-crop.pdf}    
    \end{subfigure}
    \hspace{1mm}
    \begin{subfigure}[t]{0.02\textwidth}
        \scriptsize
        \textbf{(d)}
    \end{subfigure}
    \begin{subfigure}[t]{0.4\textwidth}
        \includegraphics[width=\linewidth, valign=t]{figures/main/evolution_of_ablation-crop.pdf}    
    \end{subfigure}
    \caption{\textit{Inconsistencies in performance reports and a lack of ablation studies}. \textbf{(a)} MARL algorithms ranked by popularity. \textbf{(b)} Historical performance of QMIX on different SMAC maps across papers. \textbf{(c)} Performance of QMIX on the MMM2 SMAC map as reported in different papers. \textbf{(d)} A count of papers over the years containing any type of ablation study as part of their evaluation of a newly proposed algorithm.}
    \label{fig: smac mmm2 qmix}
\end{figure}

 \textbf{The situation in MARL} -- \textit{Similar inconsistencies and poor reporting but a promising rise in ablation studies}: There already exist some work in MARL showing the effects of specific code-level optimisations on evaluation performance \citep{hu2021rethinking}. Employing different optimisers, exploration schedules, or simply setting the number of rollout processes to be different, can have a significant effect on algorithm performance. To better understand the variance in performance reporting across works in MARL, we focused on QMIX \citep{rashid2018qmix}, the most popular algorithm in our dataset (as shown in Figure \ref{fig: smac mmm2 qmix} (a)). In Figure \ref{fig: smac mmm2 qmix} (b), we plot the performance of QMIX tested on different maps from the StarCraft multi-agent challenge (SMAC) environment \citep{samvelyan19smac}, a popular benchmark in MARL. On several maps, we find wildly different reported performances with large discrepancies across papers. Although it is difficult to pin down the exact source of these differences in reports, we zoom in with our analysis to only consider a single environment, in this case \textit{MMM2}. We find that some of the variance is explained by differences in the environment version as well as the length of training time, as shown in Figure \ref{fig: smac mmm2 qmix} (c). However, even when both of these aspects are controlled for, as well as any implementation or evaluation details mentioned in each paper, differences in performance are still observed (as seen by comparing orange and blue circles, respectively). This provides evidence that unreported implementation details, or differences in evaluation methodology account for some of the observed variance and act as confounders when comparing performance across papers (similar inconsistencies in other maps are shown in the Appendix). We finally consider studying the explicit attempts in published works at understanding the sources of algorithmic improvement through the use of ablation studies. We find that very few of these studies were performed in the earlier years of MARL (see Figure \ref{fig: smac mmm2 qmix} (d)). However, even though roughly 40\% of papers in 2021 still lacked any form of ablation study, we find a promising trend showing that ablation studies have become significantly more prevalent in recent~years. 

\textbf{Recommendations} -- \textit{Report all experimental details, release code and include ablation studies}: \cite{henderson2019deep} emphasise that for results to be reproducible, it is important that papers report \textit{all} experimental details. This includes hyperparameters, code-level optimisations, tuning procedures, as well as a precise description of how the evaluation was performed on both the baseline and novel work. It is also important that code be made available to easily replicate findings and stress test claims of general performance improvements. Furthermore, \cite{engstrom2020implementation} propose that algorithm designers be more rigorous in their analysis of the effects of individual components and how these impact performance through the use of detailed ablation studies. It is important that researchers practice diligence in attributing how the overall performance of algorithms and their underlying algorithmic behavior are affected by different proposed innovations, implementation details and code-level optimisations. In the light of our above analysis, we argue that the situation is no different in MARL, and therefore suggest the field adopt more rigorous reporting and conduct detailed ablation studies of proposed innovations.

\subsection{Lesson 2: Use standardised statistical tooling for estimating and reporting uncertainty} 

\textbf{Issue in RL} -- \textit{Results in papers do not take into account uncertainty}: We have discussed how different implementations of the same algorithm with the same set of hyperparameters can lead to drastically different results. However, even under such a high degree of variability, typical methodologies often ignore the uncertainty in their reporting \citep{colas2018random, colas2019hitchhikers, jordan2020evaluating, agarwal2022deep}. Furthermore, most published results in RL make use of point estimates like the mean or median performance and do not take into account the statistical uncertainty arising from only using a finite number of testing runs. For instance, \cite{agarwal2022deep} found that the current norm of using only a few runs to evaluate the performance of an RL algorithm is insufficient and does not account for the variability of the point estimate used. Furthermore, \cite{agarwal2022deep} also revealed that the manner in which point estimates are chosen varies between authors. This inconsistency invalidates direct comparison between results across papers. 

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.02\textwidth}
        \scriptsize
        \textbf{(a)}
    \end{subfigure}
    \begin{subfigure}[t]{0.25\textwidth}
        \includegraphics[width=\linewidth, valign=t]{figures/main/aggregate_function-crop.pdf}
    \end{subfigure}
    \hspace{1mm}
    \begin{subfigure}[t]{0.02\textwidth}
        \scriptsize
        \textbf{(b)}
    \end{subfigure}
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[width=\linewidth, valign=t]{figures/main/measure_of_spread-crop.pdf}
    \end{subfigure}
    \hspace{1mm}
    \begin{subfigure}[t]{0.02\textwidth}
        \scriptsize
        \textbf{(c)}
    \end{subfigure}
    \begin{subfigure}[t]{0.4\textwidth}
        \includegraphics[width=\linewidth, valign=t]{figures/main/evolution_measure_of_spread-crop.pdf}
    \end{subfigure}

    \vspace{0.4cm}

    \begin{subfigure}[t]{0.02\textwidth}
        \scriptsize
        \textbf{(d)}
    \end{subfigure}
    \begin{subfigure}[t]{0.29\textwidth}
        \includegraphics[width=\linewidth, valign=t]{figures/main/evolution_frequency_metric-crop.pdf}
    \end{subfigure}
    \hspace{1mm}
    \begin{subfigure}[t]{0.02\textwidth}
        \scriptsize
        \textbf{(e)}
    \end{subfigure}
    \begin{subfigure}[t]{0.29\textwidth}
        \includegraphics[width=\linewidth, valign=t]{figures/main/evolution_of_evaluation_duration-crop.pdf}
    \end{subfigure}
    \hspace{1mm}
    \begin{subfigure}[t]{0.02\textwidth}
        \scriptsize
        \textbf{(f)}
    \end{subfigure}
    \begin{subfigure}[t]{0.29\textwidth}
        \includegraphics[width=\linewidth, valign=t]{figures/main/independent_runs-crop.pdf}
    \end{subfigure}
    \caption{\textit{Trends in performance aggregation, uncertainty quantification and omissions in reporting on key aspects of evaluation methodology}. \textbf{(a)} Distribution of performance aggregation metrics. None means that the aggregation metric was not specified in the paper. \textbf{(b)} Distribution of uncertainty methods: $\alpha\%$ confidence interval (CI), standard deviation (STD) and interquartile range (IQR). \textbf{(c)} Trends in uncertainty quantification over time. \textbf{(d)} Reporting of the evaluation interval used. \textbf{(e)} Reporting on the number of evaluation runs used. \textbf{(f)} Number of independent runs used in published work.}
    \label{fig: uncertainty estimation}
\end{figure}

\textbf{The situation in MARL} -- \textit{A lack of shared standards for uncertainty estimation and concerning omissions in reporting}: In Figure \ref{fig: uncertainty estimation} (a)-(c), we investigate the use of statistical aggregation and uncertainty quantification methods in MARL. We find considerable variability in the methods used, with little indication of standardisation. Perhaps more concerning is a complete absence of proper uncertainty quantification from one third of published papers. On a more positive note, we observe an upward trend in the use of standard deviation as an uncertainty measure in recent years, particularly in 2021. Furthermore, it has become fairly standard in MARL to evaluate algorithms at regular intervals during the training phase by conducting a certain number of independent evaluation runs in the environment using the current set of learned parameters. This procedure is then followed for each independent training run and results are aggregated to assess final performance. In our analysis, we find that key aspects of this procedure are regularly omitted during reporting, as shown in Figure \ref{fig: uncertainty estimation} (d)-(e). Specifically, in (d), we find many papers omit details on the exact evaluation interval used, and in (e), a similar trend in omission regarding the exact number of independent evaluation runs used. Finally, in Figure \ref{fig: uncertainty estimation} (f), we plot the number of independent runs used during training, showing no clear standard. Given the often high computational requirements of MARL research, it is not surprising that most works opt for a low number of independent training runs, however this remains of concern when making statistical claims. 

\textbf{Recommendations} -- \textit{Standardised statistical tooling and uncertainty estimation including detailed reporting}: As mentioned before, the computational requirements in MARL research often make it prohibitively difficult to run many independent experiments to properly quantify uncertainty. One approach to make sound statistical analysis more tractable, is to pool results across different tasks using the bootstrap \citep{Efron1992}. In particular, for RL, \cite{agarwal2022deep} recommend computing stratified bootstrap confidence intervals, where instead of only using the original set of data to calculate confidence intervals, the data is resampled with replacement from $M$ tasks, each having $N$ runs. This process is repeated as many times as needed to approximate the sampling distribution of the statistic being calculated. Furthermore, when making a summary of overall performance across tasks it has been shown that the mean and median are insufficient, the former being dominated by outliers and the latter having higher variance. Instead, \cite{agarwal2022deep} propose the use of the interquartile mean (IQM) which is more robust to outlier scores than the mean and more statistically efficient than the median. Finally, \cite{agarwal2022deep} propose the use of probability of improvement scores, sample efficiency curves and performance profiles, which are commonly used to compare the performance of optimization algorithms \citep{performance_profiles}. These performance profiles are inherently robust to outliers on both ends of the distribution tails and allow for the comparison of relative performance at a glance. In the shared reward setting, where it is only required to track a single return value, we argue that these tools fit the exact needs of cooperative MARL, as they do in RL. Furthermore, in light of our analysis, we strongly recommend a universal standard in the use, and reporting of, evaluation parameters such as the number of independent runs, evaluation frequency, performance metrics and statistical tooling, to make comparisons across different works easier and more fair. 

% TODO: explain why tools fit the needs of coop MARL so well.

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.02\textwidth}
        \scriptsize
        \textbf{(a)}
    \end{subfigure}
    \begin{subfigure}[t]{0.6\textwidth}
        \includegraphics[width=\linewidth, valign=t]{figures/main/evolution_environment_more_2_mentions-crop.pdf}
    \end{subfigure}
    \hspace{1mm}
    \begin{subfigure}[t]{0.02\textwidth}
        \scriptsize
        \textbf{(b)}
    \end{subfigure}
    \begin{subfigure}[t]{0.28\textwidth}
        \includegraphics[width=\linewidth, valign=t]{figures/main/4_num_env_class_per_paper-crop.pdf}
    \end{subfigure}

    \vspace{0.4cm}

    \begin{subfigure}[t]{0.02\textwidth}
        \scriptsize
        \textbf{(c)}
    \end{subfigure}
    \begin{subfigure}[t]{0.22\textwidth}
        \includegraphics[width=\linewidth, valign=t]{figures/main/4_num_envs_per_paper-crop.pdf}
    \end{subfigure}
    \hspace{1mm}
    \begin{subfigure}[t]{0.02\textwidth}
        \scriptsize
        \textbf{(d)}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\textwidth}
        \includegraphics[width=\linewidth, valign=t]{figures/main/map_difficulty_smac-crop.pdf}
    \end{subfigure}
    \hspace{1mm}
    \begin{subfigure}[t]{0.02\textwidth}
        \scriptsize
        \textbf{(e)}
    \end{subfigure}
    \begin{subfigure}[t]{0.4\textwidth}
        \includegraphics[width=\linewidth, valign=t]{figures/main/top_win_rate.pdf}
    \end{subfigure}
    \caption{\textit{Environment popularity, usage trends in papers and potential evidence of overfitting on SMAC.} \textbf{(a)} Environment adoption over time. \textbf{(b)} Number of environments used in papers. \textbf{(c)} Number of scenarios/tasks/maps used in papers. \textbf{(d)} Distribution of task difficulty of SMAC maps used in papers. \textbf{(e)} Performance trends on popular SMAC maps: Aggregation is the aggregate function used for the different reported values.}
    \label{fig: smac env}
\end{figure}

\subsection{Lesson 3: Guard against environment misuse and overfitting}

\textbf{Issue in RL} -- \textit{Over-tuning algorithms to perform well on a specific environment}: As early as 2011 issues with evaluation in RL came to the foreground in the form of \textit{environment overfitting}. \cite{whiteson2011protecting} raised the concern that in the context of RL, researchers might over-tune algorithms to perform well on a specific benchmark at the cost of all other potential use cases. More specifically, \cite{whiteson2011protecting} define environment overfitting in terms of a desired target distribution. When an algorithm performs well in a specific environment but lacks performance over a target \textit{distribution} of environments, it can be deemed to have overfit that particular environment.

\textbf{The situation in MARL} -- \textit{One environment to rule them all -- on the use and misuse of SMAC}: The StarCraft multi-agent challenge (SMAC) \citep{samvelyan19smac} has quickly risen to prominence as a key benchmark for MARL research since it's release in 2019, rivaled only in use by the multi-agent particle environment (MPE) introduced by \cite{lowe2017multi} (see Figure \ref{fig: smac env} (a)). SMAC and its accompanied MARL framework PyMARL (introduced in the same paper), fulfills several desirable properties for benchmarking: offering multiple maps of various difficulty that test key aspects of MARL algorithms and providing a unified API for running baselines as well as state-of-the-art algorithms on SMAC. Unfortunately, the wide-spread adoption of SMAC has also caused several issues, relating to environment overfitting and cherry picking of results, putting into question the credibility of claims made while using it as a benchmark. 

To illustrate the above point, we start by highlighting that many MARL papers use only a single environment (e.g. SMAC or MPE) for evaluation, as shown in Figure \ref{fig: smac env} (b). This is often deemed acceptable since both SMAC and MPE provide many different tasks, or maps. For instance, in SMAC, there are 23 different maps providing a wide variety in terms of the number of agents, agent types and game dynamics. However, there is no standard, or agreed upon set of maps to use for benchmarking novel work, which makes it easy for authors to selectively subsample maps post-experiment based on the outcomes of their proposed algorithm. As shown in Figure \ref{fig: smac env} (c), although environments like SMAC and MPE offer many different testing scenarios, it is typical for papers to only use a small number of these in their reported experiments.

To concretely expose the potential danger in this author map selection bias, we redo the original analysis performed by \cite{samvelyan19smac}, using the authors' exact experimental data that was made publicly available\footnote{We applaud the authors for making their raw evaluation data publicly available. This data can be found here: \href{https://github.com/oxwhirl/smac}{https://github.com/oxwhirl/smac}.}, containing five independent runs for IQL \citep{tampuu2015multiagent}, COMA \citep{foerster2018counterfactual}, VDN \citep{sunehag2017value} and QMIX \citep{rashid2018qmix} on 14 SMAC maps.\footnote{The maps chosen were: 1c3s5z, 2c\_vs\_64zg, bane\_vs\_bane, MMM2, 10m\_vs\_11m, 27m\_vs\_30m, 5m\_vs\_6m, 2s3z, 2s\_vs\_1sc, s5z, 3s\_vs\_5z, 6h\_vs\_8z, 3s5z\_vs\_3s6z and corridor} The top row of Figure \ref{fig: smac re-analysis} shows the results of this analysis performed using the statistical tools recommended by \cite{agarwal2022deep}, including the probability of improvement between algorithms, performance profiles and sample efficiency curves. The results support the original claims made by \cite{samvelyan19smac}, namely that QMIX is a superior algorithm to that of VDN, COMA and IQL, both in terms of performance and sample efficiency. However, by simply sampling a smaller set of two easy, medium and hard maps (a common spread in the literature, see Figure \ref{fig: smac env} (d)), from the original 14, giving 6 maps in total (a reasonable number according to prior work, see Figure \ref{fig: smac env} (c)), we are able to change the outcome of the analysis in support of no difference in performance between VDN and QMIX, as well as finding VDN to be more sample efficient. This is shown in the bottom row of Figure \ref{fig: smac re-analysis} and highlights the danger of a lack of standards regarding which \textit{fixed} set of maps should be used for benchmarking.

\begin{figure}
    \centering
    \includegraphics[width=0.34\textwidth]{figures/main/smac_probability_of_improvement.pdf}
    \hspace{1mm}
    \includegraphics[width=0.33\textwidth]{figures/main/smac_performance_profiles.pdf}
    \includegraphics[width=0.29\textwidth]{figures/main/smac_sample_efficiency_curve.pdf}
    \includegraphics[width=0.34\textwidth]{figures/main/re_smac_probability_of_improvement.pdf}
    \hspace{1mm}
    \includegraphics[width=0.33\textwidth]{figures/main/re_smac_performance_profiles.pdf}
    \includegraphics[width=0.29\textwidth]{figures/main/re_smac_sample_efficiency_curve.pdf}
    \caption{\textit{Reanalysis of original SMAC experiments conducted by \cite{samvelyan19smac} including probability of improvement, performance profiles and sample efficiency curves}. \textbf{Top row:} All 14 SMAC maps used in the original analysis. \textbf{Bottom row:} Subset of 6 maps, including 2 easy, 2 medium and 2 hard: 2s\_vs\_1sc, 3s\_vs\_5z, bane\_vs\_bane, 5m\_vs\_6m, 6h\_vs\_8z and corridor}
    \label{fig: smac re-analysis}
\end{figure}

We end our investigation into SMAC (and refer the reader to the Appendix for additional discrepancies uncovered), by looking at historical performance trends. In Figure \ref{fig: smac env} (e), we show the top win rate achieved by an algorithm in a specific year for 14 of the most popular maps used in prior work. We find that by 2021, most of these maps have converged to a win rate close or equal to 100\%, while only a few maps are still situated around 80-90\%. Given that many of these maps repeatedly feature across papers, and will likely be used in future work, it begs the question to what extent the MARL community has already overfit to SMAC as an evaluation benchmark. 

\textbf{Recommendations} -- \textit{Standardised environment sets and testing for generalisation}: To solve the issue of environment overfitting, \cite{whiteson2011protecting} propose the use of a generalised evaluation methodology. In this approach, environments (for tuning algorithms) are freely sampled from some generalised environment set. Separately, algorithm evaluation is performed on a second set of sampled environments from the same generalised environment set, acting as a test set analogous to that used in supervised learning. Recent work in this direction include benchmarks such as Procgen \citep{cobbe2020leveraging}, which use procedural generation to implicitly construct a distribution from which to sample test tasks. In SMAC and other environments, it is common practice to only evaluate on the exact map the algorithm was trained on, under that exact same conditions, and to not specifically test for generalisation across unseen tasks. However, many MARL algorithms are still highly sensitive to small changes in the environment and often fail to generalise to new unseen tasks \citep{carion2019structured, zhang2020multi, mahajan2022generalization}. This calls for more work on MARL generalisation and we recommend a stronger focus on benchmarks designed specifically to test generaliation. However, it has been noted that procedurally generated benchmarks may reduce the precision of research \citep{kirk2021survey}, making it more difficult to track progress. Furthermore, MARL exibits several unique and challenging difficulties when it comes to building algorithms able to generalise, likely requiring many years of future work to surmount \citep{mahajan2022generalization}. Therefore, in certain cases, it might make more sense for researchers to take smaller and more precise steps towards key innovations in algorithm design by still relying on traditional environment sets. In this setting, we strongly advocate using fixed environment sets, where ideally these are selected by the designers of each environment and are accompanied by exact instruction for their configuration, so as to be consistent across papers.
\newpage

==> emarl - meta analysis 2/sections/3-protocol.tex <==
\section{Towards a standardised evaluation protocol for MARL} \label{sec: eval protocol}

In this section, we pool together the observations and recommendations from the previous section to provide a standardised performance evaluation protocol for cooperative MARL. We are realistic in our efforts, knowing that a single protocol is unlikely to be applicable to all MARL research. However, echoing recent work on evaluation \citep{ulmer2022experimental}, we stress that many of the issues highlighted previously stem from a lack of \emph{standardisation}. Therefore, we believe a default "off-the-shelf" protocol that is able capture most settings, could provide great value to the community. If widely adopted, such a standardised protocol would make it easier and more accurate to compare across different works and remove some of the noise in the signal regarding the true rate of progress in MARL research. A summarised version of our protocol is given in the blue box at the end of this section and a concrete demonstration of its usage can be found in the Appendix.

\textbf{Benchmarks and Baselines. } Before giving details on the proposed protocol, we first briefly comment on benchmarks and baselines used in experiments. These choices often depend on the research question of interest, the novel work being proposed and key algorithmic capabilities to be tested. However, as alluded to in our analysis, we recommend that environment designers take full ownership regarding how their environments are to be used for evaluation. For example, if an environment has several available static tasks, the designers should specify a fixed compulsory minimum set for experiments to avoid biased subsampling by authors. It could also be helpful if designers keep track of state-of-the-art (SOTA) performances on tasks from published works and allow authors to submit these for vetting. We also strongly recommend using more than a single environment (e.g. SMAC) and preferring environments that test generalisation. Regarding baselines, we recommend that at minimum the published SOTA contender to novel work should be included. For example, if the novel proposal is a value-based off-policy algorithm for discrete environments, at minimum, it must be compared to the current SOTA value-based off-policy algorithm for discrete environments. Finally, all baselines must be tuned fairly with the same compute budget.

\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/main/evaluation_interval-crop.pdf}

    \vspace{0.4cm}

    \includegraphics[width=0.22\textwidth]{figures/main/all_timestep-crop.pdf}
    \includegraphics[width=0.24\textwidth]{figures/main/distribution_win_rate_2s3z_per_timestep-crop.pdf}
    \caption{\textbf{Top:} Evaluation methodologies in papers: how frequent and for how many runs to do evaluation. ``E'' refers to episode and ``T'' to timestep.  \textbf{Bottom:} Number of total training timesteps used in papers (left) and win rates per training timesteps on 2s3z (right).}
    \label{fig: exp parameters}
\end{wrapfigure}

\textbf{Evaluation parameters. }  In Figure \ref{fig: exp parameters}, we show the evaluation parameters for the number of evaluation runs, the evaluation interval (top) and the training time (bottom left) used in papers. We find it is most common to use 32 evaluation episodes at every 10000 timesteps (defined as the steps taken by agents when acting in the environment) and to train for 2 million timesteps in total. We note that these numbers are skewed towards earlier years of SMAC evaluation and that recent works have since explored far longer training times. However, we argue that these longer training times are not always justified (e.g. see the bottom right of Figure \ref{fig: exp parameters}). Furthermore, SMAC is one of the most expensive MARL environments (Appendix A.7 in \citet{papoudakis2021benchmarking}) and for the future accessibility of research in terms of scale and for fair comparisons across different works, we recommend the above commonly used values as reasonable starting defaults and support the view put forward by \cite{dodge2019show} that results should be interpreted as a function of the compute budget used. We of course recognise that these evaluation parameters can be very specific to the environment, or task, and again we urge environment designers to play a role in helping the community develop and adopt sensible standards. Finally, as done by \cite{papoudakis2021benchmarking}, we recommend treating off-policy and on-policy algorithms differently and train on-policy algorithms for a factor of 10 more timesteps than off-policy algorithms due to differences in sample efficiency. As argued by \cite{papoudakis2021benchmarking}, with modern simulators, the wall-clock time of on-policy training done in this way is typically not much slower than off-policy training.

\textbf{Performance and uncertainty quantification. } To aggregate performance across evaluation intervals, we recommend using the \textit{absolute} performance metric proposed by \cite{colas2018gep}, computed using the best average (over training runs) joint policy found during training. Typically, practitioners checkpoint the best performing policy parameters to use as the final model, therefore it makes sense to do evaluation in a similar way. However, to account for not averaging across different evaluation intervals, \cite{colas2018gep} recommend increasing the number of independent evaluation runs using the best policy by a factor of 10 compared to what was used at other intervals. To quantify uncertainty, we recommend using the mean with 95\% confidence intervals (CIs) at each evaluation interval (computed over independent evaluation runs), and when aggregating across tasks within an environment, we recommend using the tools proposed by \cite{agarwal2022deep}, in particular, the inter-quartile mean (IQM) with 95\% stratified Bootstrap CIs.

\textbf{Reporting. } We strongly recommend reporting \textit{all} relevant experimental details including: hyperparameters, code-level optimisations, computational requirements and frameworks used. Taking inspiration from \textit{model cards} \citep{mitchell2019model}, we provide templates for reporting in the Appendix. Furthermore, we recommend providing experimental results in multiple formats, including plots \textit{and} tables per task and environment as well as making all raw experimental data and code publicly available for future analysis and easy comparison. Finally, we encourage authors to include detailed ablation studies in their work, so as to be able to accurately attribute sources of improvement.

\begin{mybox}{A Standardised Performance Evaluation Protocol for Cooperative MARL}
    % \textbf{1. Benchmarks}
    % \begin{itemize}
    %     \item Selection: 
    % \end{itemize}
    % \textbf{2. Baselines}
    % \begin{itemize}
    %     \item Selection: Published state-of-the-art (SOTA) contender to novel work. 
    %     \
    % \end{itemize}
    \footnotesize
    \textbf{Input: } Environments with tasks $t$ from a set $\mathcal{T}$. Algorithms $a \in \mathcal{A}$, including baselines and novel work.\\

    \textbf{1. Evaluation parameters -- defaults}
    \begin{itemize}
        \item Number of training \textit{timesteps}, $T = 2$ million (off-policy), $T= 20$ million (on-policy).
        \item Number of independent training \textit{runs}, $R = 10$ (from \cite{agarwal2022deep})
        \item Number of independent evaluation \textit{episodes} per interval, $E = 32$.
        \item Evaluation \textit{intervals}, $i \in \mathcal{I}$, at every 10000 timesteps.
        % \item Hyperparameters: For each environment optimise all algorithms fairly (e.g. using grid search with a fixed compute budget). At minimum, do this for a single task and then use these for all others tasks in that environment.
    \end{itemize}
    \textbf{2. Performance and uncertainty quantification}
    \begin{enumerate}
        \item Performance metric: Always use returns $G$ (applicable to all environments), \emph{and} the environment specific metric (e.g. Win rate).
        \item Per task evaluation: Compute the mean $G^a_t$ over $E$ episodes at each evaluation interval $i$, where $G^a_t$ is the return of algorithm $a$ on task $t$, with 95\% CI, for all $a$.
        \item Per environment evaluation: 
        \begin{itemize}
            \item Compute the normalised \emph{absolute} return \citep{colas2018gep} as the mean return of $10\times E = 320$ evaluation episodes using the best joint policy found during training and normalising the return to be in the range $[0,1]$ using $(G^a_t - \min(G_t))/(\max(G_t)-\min(G_t))$, where $G_t$ is the return for all algorithms on task $t$. 
            \item For each algorithm $a$, form an evaluation matrix with shape $(R, |\mathcal{T}|)$ where each entry is the normalised absolute return for a specific training run on a specific task. 
            \item Compute the IQM and optimality gap with 95\% stratified Bootstrap CIs, probability of improvement scores and performance profiles, to compare the algorithms, using the tools proposed by \cite{agarwal2022deep}.\footnote{\scriptsize These can be found in the \texttt{rliable} library: \href{https://github.com/google-research/rliable}{https://github.com/google-research/rliable}} Sample efficiency curves can be computed by using normalised returns at each evaluation interval.
        \end{itemize}
        % \item Ablation study of key components using (4.2-4.3).
    \end{enumerate}
    \textbf{3. Reporting}
    \begin{itemize}
        \item Experiments: All hyperparameters, code-level optimisations, computational requirements and framework details.
        \item Plots: All task and environment evaluations as well as ablation study results.
        \item Tables: Normalised absolute performance per task with 95\% CI for all tasks, IQM with 95\% stratified Bootstrap CIs per environment for all environments.
        \item Public repository: Raw evaluation data and code implementations.
    \end{itemize}
\end{mybox}





% \begin{figure}
%     \centering
%     \begin{subfigure}[t]{0.02\textwidth}
%         \scriptsizes
%         \textbf{(a)}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.4\textwidth}
%         \includegraphics[width=\linewidth, valign=t]{figures/main/all_timestep-crop.pdf}
%     \end{subfigure}
%     \hspace{1mm}
%     \begin{subfigure}[t]{0.02\textwidth}
%         \scriptsize
%         \textbf{(b)}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.4\textwidth}
%         \includegraphics[width=\linewidth, valign=t]{figures/main/evaluation_interval-crop.pdf}
%     \end{subfigure}
%     \caption{\textit{Environment popularity, usage trends in papers and potential evidence of overfitting on SMAC.} \textbf{(a)} Environment adoption over time. \textbf{(b)} Number of environments used in papers. \textbf{(c)} Number of scenarios used in papers. \textbf{(d)} Distribution of task difficulty of SMAC maps used in papers. \textbf{(e)} Performance trends on popular SMAC maps.}
    
% \end{figure}
    
    % \begin{table}
    %     \centering
    %     \caption{Suggested reporting tables.}
    %     \label{tab: reporting rubic for algorithms}
    %     \resizebox{0.49\columnwidth}{!}{
    %     \begin{tabular}{@{}llll@{}}
    %     \toprule
    %     Hyperparameters & Environment A  & Environment B\\
    %     \midrule
    %     Optimiser (type, parameters) &  &  \\
    %     Learning Rate &  &  \\
    %     Batch size (value, type) &  &  \\
    %     Replay Size &  &  \\s
    %     N step return, $Q(\lambda)$, $TD(\lambda)$ &  &  \\
    %     Entropy coefficient &  &  \\
    %     $\epsilon$ annealing steps s&  &  \\
    %     Policy network (input, size, type, initialisation) &  &  \\
    %     Critic network (input, size, type, initialisation) &  &  \\
    %     Mixing network (input, size, type, initialisation) &  &  \\
    %     Parameter sharing &s  &  \\
    %     $\epsilon$ during evaluation &  &  \\
    %     \midrule
    %     Code-level optimisations & & \\
    %     \midrule
    %     Value function clipping &  &  \\
    %     Value normalisation &  &  \\
    %     Reward scaling/normalisation &  &  \\
    %     Reward clipping &  &  \\
    %     Observation normalisation &  &  \\
    %     Gradient clipping &  &  \\ 
    %     Target network update (value, type) &  &  \\
    %     Layer scaling  &  &  \\
    %     Rollout processes &  &  \\
    %     \bottomrule
    %     \end{tabular}
    %     }
    %     \resizebox{0.49\columnwidth}{!}{
    %     \begin{tabular}{@{}llll@{}}
    %         \toprule
    %         Settings &  Task A  & Task B \\
    %         \midrule
    %         Difficulty (type, parameters) & value for A & Value for B \\
    %         Total number of agents & value for A & Value for B \\
    %         Agent types and numbers & value for A & Value for B \\
    %         Full state space & value for A & Value for B \\
    %         Local observation space & value for A & Value for B \\
    %         Action space & value for A & Value for B \\
    %         Reward & value for A & Value for B \\
    %         Dead agent handling & value for A & Value for B \\
    %         End of episode criteria & value for A & Value for B \\
    %         Random baseline performance & value for A & Value for B \\
    %         Prior SOTA performance (paper, algorithm) & value for A & Value for B \\
    %         \bottomrule
    %         \end{tabular}
    %     }
    % \end{table}
    

% \begin{itemize}
%     % \item List all hyperparemeters, code-level optimisations and environment settings -> show table
%     % \item Include tables as well as plots
%     % \item Make all raw evaluation data publicly available
%     % \item Specify framework and make code publicly available
%     % \item Use appropriate statistical tooling -> suggest rliable metrics and tools
%     % \item Standardise aggregation methodology, metric, step count and training time
%     \item Standardise (subset of) maps per environment, version and other settings -> ideally from designers (can be sensibly adjusted over time) - Fixed task set, should not be up to the discretion of the authors to choose which environments to use. 
%     \item Prefer environments that test generalisation and not overfitting
%     % \item fix the number of seeds (10), evaluation interval (get from data), number of eval runs (from data)
%     % \item Aggregation: Always use two - mean over all eval runs across training, and Max (same as benchmarking paper).
%     % \item For independent variable, use timesteps.
% \end{itemize}

% \begin{table}
%     \centering
%     \caption{Reporting rubric for Algorithm A}
%     \label{tab: reporting rubic for algorithms}
%     \begin{tabular}{@{}llll@{}}
%     \toprule
%     Environments & Environment A  & Environment B  \\ 
%     \midrule
%     Hyperparameters & & \\
%     \midrule
%     Optimiser (type, parameters) & value for A & Value for B \\
%     Learning Rate & value for A & Value for B \\
%     Batch size (value, type) & value for A & Value for B \\
%     Replay Size & value for A & Value for B \\
%     N step return, $Q(\lambda)$, $TD(\lambda)$ & value for A & Value for B \\
%     Entropy coefficient & value for A & Value for B \\
%     $\epsilon$ annealing steps & value for A & Value for B \\
%     Policy network (input, size, type, initialisation) & value for A & Value for B \\
%     Critic network (input, size, type, initialisation) & value for A & Value for B \\
%     Mixing network (input, size, type, initialisation) & value for A & Value for B \\
%     Parameter sharing & value for A & Value for B \\
%     \midrule
%     Code-level optimisations & & \\
%     \midrule
%     Value function clipping & value for A & Value for B \\
%     Value normalisation & value for A & Value for B \\
%     Reward scaling/normalisation & value for A & Value for B \\
%     Reward clipping & value for A & Value for B \\
%     Observation normalisation & value for A & Value for B \\
%     Gradient clipping & value for A & Value for B \\ 
%     Target network update (value, type) & value for A & Value for B \\
%     Layer scaling  & value for A & Value for B \\
%     \midrule
%     Evaluation settings & & \\
%     \midrule
%     Rollout processes & value for A & Value for B \\
%     Evaluation interval & value for A & Value for B \\
%     Number of evaluation runs & value for A & Value for B \\
%     Number of seeds (independent runs) & value for A & Value for B \\
%     $\epsilon$ during evaluation & value for A & Value for B \\
%     \bottomrule
%     \end{tabular}
% \end{table}

% \begin{table}
%     \centering
%     \caption{Reporting rubric for Environment A (version x.x)}
%     \label{tab: reporting rubic for algorithms}
%     \begin{tabular}{@{}llll@{}}
%     \toprule
%     Scenarios &  Scenario A  & Scenario B \\ 
%     \midrule
%     Settings & & \\
%     \midrule
%     Difficulty (type, parameters) & value for A & Value for B \\
%     Total number of agents & value for A & Value for B \\
%     Agent types and numbers & value for A & Value for B \\
%     Full state space & value for A & Value for B \\
%     Local observation space & value for A & Value for B \\
%     Action space & value for A & Value for B \\
%     Reward & value for A & Value for B \\
%     Dead agent handling & value for A & Value for B \\
%     End of episode criteria & value for A & Value for B \\
%     Random baseline performance & value for A & Value for B \\
%     Prior SOTA performance (paper, algorithm) & value for A & Value for B \\
%     % \midrule
%     % Code-level optimisations & & \\
%     % \midrule
%     % Value function clipping & value for A & Value for B \\
%     % Value normalisation & value for A & Value for B \\
%     % Reward scaling/normalisation & value for A & Value for B \\
%     % Reward clipping & value for A & Value for B \\
%     % Observation normalisation & value for A & Value for B \\
%     % Gradient clipping & value for A & Value for B \\ 
%     % Target network update (value, type) & value for A & Value for B \\
%     % Layer scaling  & value for A & Value for B \\
%     % \midrule
%     % Evaluation settings & & \\
%     % \midrule
%     % Rollout processes & value for A & Value for B \\
%     % Evaluation interval & value for A & Value for B \\
%     % Number of evaluation runs & value for A & Value for B \\
%     % Number of seeds (independent runs) & value for A & Value for B \\
%     % $\epsilon$ during evaluation & value for A & Value for B \\
%     \bottomrule
%     \end{tabular}
% \end{table}



% % \begin{comment}
% % Define the search strategy\\
% % Filtration of relevant studies\\
% % Introduce annotations\\
% % Highlight considerations \\
% % Abstraction of data and setting up our own table\\
% % Data extraction\\
% % \end{comment}



% \subsubsection{Analysis}

% In the early years, there was a lack of multi-agent environments, and most publications tested their studies on environments created by the authors (paper-specific environments) and MazeBase, since it was developed for single-agent environments but it is easily adapted to multi-agent scenarios, as was performed in to create a traffic junction tasks and Combat. Since 2017, we've seen an increase in the use of MPE tasks like Predator-Prey and Spread, as well as StarCraft unit micromanagement. MPE was the most commonly utilized environment in 2019, accounting for 5 over 13 papers. However, since 2020, we see SMAC dominating with a large number of papers, making it the most used environment since 2020 to the present.

% We have classified the scenarios in SMAC based on the distribution of the win rate values across all algorithms and regardless all of the extra parameters (training time, random seed, environment settings...) and we find n easy scenarios, m medium scenarios and h hard scenarios. Although we noticed some disagreement between what we believe is an easy scenario and what is stated in certain papers as a difficult scenario, this was for a reason: e.g. 2c\_vs\_64zg is considered as a hard task in 7 out of 22 papers which is expected given that in the early years most of the algorithm performance in this scenario is under 25\% as a win rate, and one of the reasons in the increase of the win rate is the training time which has increased through the years, we find that before 2M time-steps, the results were stacked under 60\% and since 2020, the time-steps value for 2c\_vs\_64zg have gotten higher than 2M, which affect the results to reach almost 100\% regardless of the environment settings and the experiment implementation in all the collected data.
% Despite that we have n hard scenarios, most of them are used only once or twice over the 114 papers except for 6h\_vs\_8z (21 papers) and corridor (16 papers).





% \subsection{Evaluation procedure}

% The evaluation procedure has various options and details that are essential to demonstrate the experiment in each study, so that the readers have a clear understanding of the experiment if they want to reproduce it or compare it to other studies. In this section, we discuss the most important variables that are required and must be wisely chosen in an evaluation procedure of a study based on many factors such as the environment of the experiment (other factors...), as well as their alternatives depending on an analysis of what is occurring.

% \subsubsection{Metrics}
% In general, metrics are used to monitor and quantify a model's performance. In our analysis, we identify 24 employed metrics, and after unifying, based on our annotations for A3, we obtain 12
% metrics. We observe dependencies between the choice of the environment and metrics: e.g. Out of the collected SMAC data 88.3\% use \emph{Win Rate} as a metric, meanwhile in MPE, out of 1136 collected data related to MPE environment, we have 48\% use \emph{Reward} and 37.7\% of them use \emph{Return}, which begs the question, \textbf{is this dependency inevitable}, especially that out of 29 environments, we find 20 environments use one only metric type, 7 use 2 metrics and only 2 environments use plus 2 metrics.
% Moreover, we find that Win Rate represents 49.3\% of our data and is used in 43 papers we can't deny that it is the wide used metric because win rate is mostly attached to SMAC and Traffic Juction, and since these two environments are the most used environments we can confirm why we have this huge number of papers that use win rate, besides out of 29 environments, we find Win Rate is used  in different 14 environments making it the most used metric across the environments, followed by Return in 12 environments and Reward in 10 environments.

% \subsubsection{Independent runs}
% Independent training runs could take place across different random seeds or a fixed number of them, referred to as run per seed, in which some experiments take place for a specified set of random seeds with a given number of runs per seed. Fixing the random seed is an attempt to control some of the experiment's sources of randomness. The number of runs is important in determining the reliability of the evaluation, notably, the higher the number of runs per task, the lower the uncertainty and the more accurate the estimations.\\
% The authors used to employ 20 to 10 runs in the Unit Micromanagement version for the StarCraft environment, but since StarCraft II (SMAC) emerged, they tend to use 5 runs within it, and this decline may be due by the environment being more computationally costly.



% \subsubsection{Aggregate function }
% An aggregate function, also known as a measure of central tendency, is a single value that intends to portray the algorithm performance results by determining the central position among the various algorithm result obtained.
% The result of MARL algorithms is often reported with a point estimate of task performance metric, such as \textbf{Mean} and \textbf{Median} performance across tasks, aggregated over the independent training runs. The Mean is the most often used aggregation function, accounting for over 35\% of all data gathered, and it was the only utilized aggregate function in the early years, but since 2019, we have seen the introduction of the Median as an aggregate function, with the launch of SMAC, and it has became one of the most widely used aggregate functions in SMAC, with some exceptions in MPE.

% \subsubsection{Measure of spread}

% The measure of spread plays an important role in delivering first hand information about the experiment findings. It expresses how far apart values are in the distribution or how distinct one value is from another of the metric values obtained across different random seeds or runs.\\
% In our study, we discovered that 23 out of 65 studies did not mention the measure of spread at all, and 11 papers did not address it for at some part of their experiment for one of two reasons: The authors didn't use measure of spread which is mostly when we test over only one run, or lack of details within the paper. In statistics, there are various fundamental measures of spread, the following are the most often encountered in MARL studies:

% \textbf{Standard deviation: }is a common measure of the results' dispersion. The std will be modest if the results is clustered together. If the results is widely dispersed, the standard deviation will be considerable. t was used in 21 studies, and it is also the most popular in MPE, accounting for nearly 31.1\% of the MPE gathered data.

% \textbf{Confidence interval (CI): }(CI: for a finite-sample score can be interpreted as an estimate of plausible values for the true score. A $\alpha \times 100\%$ CI computes an interval such that if we rerun the experiment and construct the CI using a different set of runs, the fraction of calculated CIs, which would differ for each set of runs, that contain the true score would tend towards $\alpha \times 100\%$, where $\alpha \in$ [0, 1] is the nominal coverage rate. 95\% CIs are typically used in practice). It is the second most commonly employed measure as it was used in 15 papers, and we note that 95\% confidence interval is the widely used measure in CI.

% \textbf{Inter-quartile range: }has the advantage of not being impacted by outliers and is important when the researchers want to know where the majority of the findings fall. It is used in 7 papers and it is commonly used in SMAC presenting 36\% of the SMAC collected data. 

% \subsubsection{Time Measurement}
% \textbf{Independent Variable:} The training and testing time is a vital feature that must be stated by the author for a fair comparison of studies; yet, although its relevance, we notice that 7 papers lacks this information. We identified 8 options to define the independent experiment variable, but the most commonly used measure is \emph{Time-step}, which is employed in 39 papers, followed by \emph{Episode}, that accounts for 14 studies. We discover an imbalance in the use of the kinds within independent experiment variables based on the environment, with 93.9\% of SMAC collected data using Time-step as an independent variable and 42.5\% of MPE collected data using Episodes.

% \textbf{Evaluation Frequency: }is generally associated with the SMAC evaluation protocol; it refers to suspending training after each set of duration T to test the algorithm for different particular duration E and running agents executing action selection,  commonly, greedily in a decentralized method. The test win rate is the percentage of E in which the agents defeat all enemy units within the time limit. Although it is predominantly employed in SMAC experiments within 12 papers  out of the 32 papers that use this environment, this evaluation approach is also used in MPE within 4 studies and in Level-Based Foraging (LBF) within 2 papers. The Evaluation Frequency must be associated with a a duration E that we recorded it as the Evaluation Duration.

% \textbf{Evaluation Duration: }as the name indicates, this is the amount of time it takes to measure an algorithm's performance; this detail is required if we have evaluation frequency, but it may be provided individually and is highly valuable. In our analysis, We noticed that n of the papers mention evaluation duration individually, and m of the publications do not include it while addressing evaluation frequency.

% % \subsection{Algorithm Comparison}

% \subsection{Pitfalls and major trends}
% % \begin{comment}
% % Open discussion of issues (general issues and issues mentioned in analysis section)
% % \end{comment}
% In this section, we discuss the findings from the analysis part by identifying six major evaluation's pitfalls such as naming conventions and lack of implementation details. Through our discussion, we report how frequently they affected publications and recent trends. Since these tendencies are important for solving existing difficulties, they may also provide a direction for future research.
% \subsection{Acceptance/Rejection criteria}
% We recorded papers from various conferences, whether they were accepted or not, since we want to raise community awareness of the limitations of the existing evaluation procedure and the reproducibility challenges. During our analysis, we collected n papers submitted to the ICLR conference, with m of them being approved, k papers from NeurIPS conference, with l approved ones...\\
% Reasons why some papers being accepted\\
% Reasons why some papers being rejected
% \subsection{Naming conventions}
% % \begin{comment}
% % Comment about naming conventions - 1. distortion of novelty in algorithms by renaming when not much novelty is added sometimes. 2. Some names add in details which specify implementation details, even though implementation detail is common to other algo's. 
% % Useful to specify where in the taxonomy of MARL algorithms your algorithm falls.
% % Jargon needs to be standardized. Papers use different words to explain the same concepts like team performance = global reward = team reward.
% % \end{comment}
% Since MARL arose in such a short amount of time, there was insufficient time to negotiate on significant norms and Jargon standardization. This lack of standardization is a crucial issue to be addressed in the field, primarily because it can lead to misunderstandings regarding experiment implementation specifics and even duplication of efforts without the algorithm creators' awareness.

% \textbf{Metrics: } From the recorded results there are a number of metrics reported which go under different names despite reporting the same information. For example, most papers make use of the reward or winrates as reportable metrics. The interpretation of winrates and rewards do not create confusion as they are a common metric in literature. However, many papers refer to scores, performance or other non-standard jargon in place of standardised terminology. 

% \textbf{Algorithms: }(we need to highlight some examples from the table that Siddarth did)

% \subsection{Lack of implementation details}
% % \begin{comment}
% % The papers don’t provide a standardized way to evaluate (e.g.: Same metric but different settings (for example: win rate but some of the mean test rate other median test rates...)
% % \end{comment}
% As we have mentioned in section 3.3, the implementation details should be provided in a paper in order for the evaluation findings to be more understandable. In the analysis, we discovered that n papers did not mention the aggregation function (u\% of all data), m papers did not address the random seed (v\%), k papers did not specify the measure of spread (h\%), and l papers did not state the independent variable (w\%). And, as seen in the figure 1, we assume that this deficiency of the details has been decreasing over years, yet it still exists.

% We consider the evaluation duration as highly important detail to be mentioned in a paper, even if the publisher does not employ evaluation frequency or has an other means of evaluating, such as average metric or final metric. As shown in the figure, we have a small number of papers mentioning this detail, which is very significant alerts, especially for the researchers who provide tabular results or evaluation curve plot instead of a training curve plot, since we only have n papers providing tabular results and exclude this detail out of all the m papers that report findings in table.

% % \begin{comment}
% % As stated in the evaluation procedure subsection, the researchers supply an aggregate function over the different runs; however, within a single run, we have another aggregation of the results, and this detail is attached to the general metric to provide more info about the used metric: e.g. Mean Reward, Mean Return and Maximum Reward. In our analysis, over 50\% of the papers that have Return as a metric they record it as the Mean Return and 3\% were just recording it as Return without details. However, this is not the case for Reward, 36\% of the recording is just Reward and even if we look for the aggregation details in these papers 77.5\% of the collected data did not provide the aggregation function.
% % \end{comment}


% The independent runs are one of the most ambiguous details cited by researchers as we need to clarify that a run might differ from utilizing a fixed random seed (run per seed), where the independent runs could refer to the number of various random seeds. We identified n publications that provided independent runs without citing the actual meaning behind it, which is something that researchers should consider in the future works.


% %Smac versions

% \subsection{Standardized environment setting}
% % \begin{comment}
% % - Smac versions differences
% % - analysis about which one is used
% % - the importance of mentioning the version (distribution of the results)
% % We can call for a unified standard set of environment configurations to be used across the most popular benchmarks. Algorithms should be allowed for a set amount of steps, random seeds need to be predetermined and used by all research groups. For MPE environment configs like the number of agents need to be fixed. Maybe some sort of global research bank of parameter configs? The flatland challenge has an example of this where a set of environment configs are given and set evaluation criteria are given as well. 
% % \end{comment}

% \subsection{The Disappearing Statistical Significance Testing}
% % \begin{comment}
% % Importance of statistical tests and the lack of their use in MARL: While the importance of statistical significance testing is regularly debated by the scientific community (Wasserstein et al., 2019), it remains one of the most cost-effective tools to check how trustworthy a particular difference between two metric scores is.
% % We can call for statistical tests to be done between algorithmic performance. Especially when improved performance is claimed. A suspected reason why this is not done is that it is computationally expensive to run, for example, 10 seeds per algorithm to obtain arrays of results for which a t-test can be performed. 
% % \end{comment}
% % Lack of testing methods: How statistical tests could be used for RL, is there any examples?

% Since the MARL researchers avoided statistical testing mostly due to computational costs, a very close option to ensuring accurate results was to indicate the statistical uncertainty, particularly for tabular data, by employing measures of spread and recording margin of error. Despite the importance of margin of error for reliable results, we identified that only 34 of the 69 papers with tabular results include it, accounting for nearly half of the recorded publications.
% \subsection{Reporting results:}
% % \begin{comment}
% % Tabular vs Plots 
% % the prob with the colors in plots...
% % \end{comment}
% %the importance of tabular results
% The recording of the experiment's findings in a table can offer readers with a complete picture of the algorithms' performance as well as a summary of the evaluation results without having to browse through the entire training phase in the plot. In our study, there are 69 articles that provide tabular and perhaps graphed findings for the experiment and 45 papers that provide completely graphed results. Despite the fact that less than the half of the studies did not provide tabular results, the number is still important and this is a warning signal because result plots, on one hand, cannot be neglected because they not only illustrate an algorithm's performance but also provide us an estimate of how long it took for the algorithm to converge. However in the other hand, if a reader requests exact values from the plot, we anticipate difficulties, for example, one of the most challenging aspects that we face while recording the results from publications is delivering accurate results from our observations to the plots, which we strongly suspect are uncertain.\\ 
% There are a variety of reasons why interpreting, reading, and recording plot findings is often challenging. Firstly, the color shading in the plot can be misleading, especially if there are multiple algorithm performances in one graph, which should be avoided, for example, in our analysis, we found a paper with a plot that illustrated the outcomes of nine algorithms in one graph, and with the close coloring shades in the graphs, it was perplexing.



% %add here aggregated suggestions from survey paper

% \section{Towards a standardised evaluation protocol for MARL}

% A guideline for MARL evaluation

% \begin{itemize}
%     \item Representation of data 
% Standardise how data is presented. Too many papers have a combination of tables and graphs that are either redundant or display an excessive amount of uninformative information. Results also need to be interpretable purely from the main body of work and should not require using the appendix to circumvent page count.

% There are evaluation protocols that are suggested by Henderson et al. (2017) and Colas et al. (2018). These papers introduce ideas called the final metric and the absolute metric. The final metric is the average over the last 100 evaluation episodes where evaluation is performed for 10 episodes at a time at fixed training intervals. The absolute metric is the average of the best policy found during training for 100 episodes. These metrics should always be computed in a separate evaluation setting where policy parameters are frozen and no training takes place.

% Making all your runs on the same graphs in slightly different shades of the same colour should be illegal. Graphs should also start at 0 if used to present results as they provide a misleading sense of scale at first glance otherwise.

% Recommend larger plots for viewing results - not small plots, also tabulated results. Can all be in appendix.
%     \item Make suggestion to include implementation details eg: network choices
% \end{itemize}

% % add in aggregated suggestions from survey paper

% % In order to mitigate sporadic evaluation in MARL as a the SMAC benchmark \citep{samvelyan19smac} suggest an evaluation procedure to be followed when using the SMAC benchmark. This evaluation procedure requires periodic greedy policy evaluation and can be done as follows: 

==> emarl - meta analysis 2/sections/4-conclusion.tex <==
\section{Conclusion and future work}

In this work, we argue for the power of standardisation. In a fast-growing field such as MARL, it becomes ever more important to be able to dispel illusions of rapid progress, potentially misleading the field and resulting in wasted time and effort. We hope to break the spell by proposing a sensible standardised performance evaluation protocol, motivated in part by the literature on evaluation in RL, as well as by a meta-analysis of prior work in MARL. If widely adopted, such a protocol could make comparisons across different works much faster, easier and more accurate. However, certain aspects of evaluation are better left standardised outside of the control or influence of authors, such as protocols pertaining to the use of benchmark environments. We believe this is an overlooked issue and an important area for future work by the community, and specifically environment designers, to jointly establish better standards and protocols for evaluation and environment use. Finally, we encourage the community to move beyond the use of only one or two environments with static task sets (e.g. MPE and SMAC) and focus more on building algorithms, environments and tools for improving generalisation in MARL.

A clear limitation of our work is our focus on the cooperative setting. Interesting works have developed protocols and environments for evaluation in both the competitive and mixed settings \citep{omidshafiei2019alpha,rowland2019,leibo2021scalable}. We find this encouraging and argue for similar efforts in the adoption of proposed standards for evaluation.
% TODO: Stress the limitation of the work here.



==> emarl - meta analysis 2/sections/8-ack.tex <==
\begin{ack}
The authors would like to kindly thank the following people for useful discussions and feedback on this work: Jonathan Shock, Matthew Morris, Claude Formanek, Asad Jeewa, Kale-ab Tessera, Sinda Ben Salem, Khalil Gorsan Mestiri, Chaima Wichka and Sasha Abramowitz.
\end{ack}

==> sections/10-checklist.tex <==
\section*{Checklist}

\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
  \answerYes{}
  \item Did you describe the limitations of your work?
  \answerYes{We did this both in our introduciton and conclusion.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{We did not find this necessary given the nature of the work.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
  \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
      \item Did you state the full set of assumptions of all theoretical results?
  \answerNo{}
      \item Did you include complete proofs of all theoretical results?
    \answerNo{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
  \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
  \answerYes{See supplementary material.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{In main text and for experiments in supplementary material.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
   \answerYes{See supplementary material.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
  \answerNo{Links to repositories were given where the license can be found.}
  \item Did you include any new assets either in the supplemental material or as a URL?
  \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
  \answerNo{All collected data is publicaly available, accesilble via open-access publication.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
  \answerNo{The meta-analysis data contains information typical to any research meta-analysis, including author information, paper titles and information extracted from each paper.}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
  \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
  \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
  \answerNA{}
\end{enumerate}


\end{enumerate}
